Reevaluation of Inductive Link Prediction

Within this paper, we show that the evaluation protocol currently used for inductive link prediction is heavily flawed as it relies on ranking the true entity in a small set of randomly sampled negative entities. Due to the limited size of the set of negatives, a simple rule-based baseline can achieve state-of-the-art results, which simply ranks entities higher based on the validity of their type. As a consequence of these insights, we reevaluate current approaches for inductive link prediction on several benchmarks using the link prediction protocol usually applied to the transductive setting. As some inductive methods suffer from scalability issues when evaluated in this setting, we propose and apply additionally an improved sampling protocol, which does not suffer from the problem mentioned above. The results of our evaluation differ drastically from the results reported in so far.

==> figures/indtrans_copy.tex <==
\begin{tikzpicture}[]

\begin{scope}[every node/.style={}]
    \node (g1) at (-0.5,-1.8) {Train/Test graph};
    \node (g2) at (3.7, -1.8) {Train graph};
    \node (g2) at (7.5, -1.8) {Test graph};
\end{scope}

%\begin{scope}[every node/.style={rectangle,draw}]
%    \node[text width=4.1cm,align=center] (g1) at (0.0,2.0) {Transductive link prediction};
%    \node[text width=4.1cm,align=center] (g2) at (5.7, 2.0) {Inductive link prediction};
%\end{scope}

% *************** TRANSDUCTIVE: TRAIN GRAPH **********************************

\begin{scope}[shift={(-1.5,1.5)}]
\draw[fill=violet!50] (0,0) circle (0.75cm);
\draw[pattern={crosshatch},pattern color=teal!50] (0,0) circle (0.75cm);
\draw[fill=blue!70] (0,0) --  (40:0.75) arc(40:80:0.75) -- cycle;
\draw[fill=red!70] (0,0) --  (0:0.75) arc(0:40:0.75) -- cycle;
\draw[color=white, rotate=3, postaction={decorate, decoration={text along path, raise=1pt,  ,text align={align=right}, text={|\tiny|training + inference \ \ \ valid \ test}, reverse path}}] (0,0) circle (0.8cm);
\end{scope}

\begin{scope}[shift={(0,0)}, every node/.style={circle,draw, inner sep=2pt, fill=white}]
\draw
(-0.5,0.9) node(a1){} (0.0,1.1) node(a2){} (0.5,1.0) node(a3){}
(-0.75,0.5) node(b1){} (-0.25,0.5) node(b2){} (0.25,0.4) node(b3){} (0.75,0.5) node(b4){}
(-1.0,0.0) node(c1){} (-0.5,0.1) node(c2){} (0.0,0.0) node(c3){} (0.5,-0.2) node(c4){} (1.0,0.0) node(c5){}
(-0.75,-0.5) node(d1){} (-0.25,-0.5) node(d2){} (0.2,-0.4) node(d3){} (0.75,-0.5) node(d4){}
(-0.6,-1.0) node(e1){} (0.0,-1.2) node(e2){} (0.6,-1.0) node(e3){};

% \draw[black, line cap=butt, line width=2pt] (a3) -- (a4); \draw[yorange!80, line width=1pt] (a3) -- +(a4);

\draw[violet!50, line width=2pt] (b1) -- (a1) -- (b2) -- (a2) -- (b3) -- (a3) -- (b4);
\draw[teal!50, line width=2pt, dotted] (b1) -- (a1) -- (b2) -- (a2) -- (b3) -- (a3) -- (b4);
\draw[violet!50, line width=2pt] (e1) -- (d1) -- (e2) -- (d2) -- (e2) -- (d3) -- (e2);
\draw[teal!50, line width=2pt, dotted] (e1) -- (d1) -- (e2) -- (d2) -- (e2) -- (d3) -- (e2);
\draw[teal!50, line width=2pt] (b1) -- (c1) -- (c2) -- (c3) -- (b3) -- (c4) -- (c5);
\draw[violet!50, line width=2pt, dotted] (b1) -- (c1) -- (c2) -- (c3) -- (b3) -- (c4) -- (c5);
\draw[teal!50, line width=2pt] (e3) -- (d4) -- (c5);
\draw[violet!50, line width=2pt, dotted] (e3) -- (d4) -- (c5);
\draw[teal!50, line width=2pt] (c1) -- (d1);
\draw[violet!50, line width=2pt, dotted] (c1) -- (d1);
\draw[blue!70, line width=2pt] (b4) -- (c4);
\draw[blue!70, line width=2pt] (e1) -- (e2);
\draw[blue!70, line width=2pt] (b1) -- (c2);
\draw[red!70, line width=2pt] (c1) -- (d1);
\draw[red!70, line width=2pt] (a2) -- (a3);
\draw[red!70, line width=2pt] (d3) -- (d4);

\end{scope}

\draw[line width=1pt] (2,2.5) -- (2,-2.0) ;

% *************** INDUCTIVE: TRAIN GRAPH **********************************


\begin{scope}[shift={(3.5,1.5)}]
\draw[fill=teal!50] (0,0) circle (0.75cm);
\draw[fill=blue!70] (0,0) --  (0:0.75) arc(0:40:0.75) -- cycle;
\draw[color=white, rotate=3, postaction={decorate, decoration={text along path, raise=1pt,  ,text align={align=right}, text={|\tiny|training \ \ \ valid}, reverse path}}] (0,0) circle (0.8cm);
\end{scope}

\begin{scope}[shift={(4.0,-0.7)}, every node/.style={circle,draw, inner sep=2pt, fill=white}]
\draw
(-0.5,0.9) node(a1){} (0.0,1.1) node(a2){} (0.5,1.0) node(a3){}
(-0.75,0.5) node(b1){} (-0.25,0.5) node(b2){} (0.25,0.4) node(b3){} (0.75,0.5) node(b4){}
(-1.0,0.0) node(c1){} (-0.5,0.1) node(c2){} (0.0,0.0) node(c3){} (0.5,-0.2) node(c4){};

\draw[teal!50, line width=2pt] (a1) -- (b2) -- (a2) -- (b3) -- (a3) -- (b4);
\draw[teal!50, line width=2pt] (b1) -- (c1) -- (c2) -- (c3) -- (b3);
%\draw[teal!50, line width=2pt] (e3) -- (d4) -- (c5);
%\draw[teal!50, line width=2pt] (c1) -- (d1);
\draw[teal!50, line width=2pt] (b4) -- (c4);
\draw[teal!50, line width=2pt] (b1) -- (c2);
\draw[teal!50, line width=2pt] (a2) -- (a3);
\draw[blue!50, line width=2pt] (b1) -- (a1);
\draw[blue!50, line width=2pt] (b3) -- (c4);

\end{scope}


% *************** INDUCTIVE: TEST GRAPH **********************************
\begin{scope}[shift={(7.5,1.5)}]
\draw[fill=violet!50] (0,0) circle (0.75cm);
\draw[fill=red!70] (0,0) --  (0:0.75) arc(0:40:0.75) -- cycle;
\draw[color=white, rotate=3, postaction={decorate, decoration={text along path, raise=1pt,  ,text align={align=right}, text={|\tiny|inference \ \ \ test}, reverse path}}] (0,0) circle (0.8cm);
\end{scope}


\begin{scope}[shift={(7.8,0.4)}, every node/.style={circle,draw, inner sep=2pt, fill=white}]
\draw
(1.0,0.0) node(c5){}
(-0.75,-0.5) node(d1){} (-0.25,-0.5) node(d2){} (0.2,-0.4) node(d3){} (0.75,-0.5) node(d4){}
(-0.6,-1.0) node(e1){} (0.0,-1.2) node(e2){} (0.6,-1.0) node(e3){};
\draw[violet!50, line width=2pt] (e1) -- (d1) -- (e2) -- (d2) -- (e2) -- (d3) -- (e2);
\draw[violet!50, line width=2pt] (e1) -- (d1) -- (e2) -- (d2) -- (e2) -- (d3) -- (e2);
\draw[violet!50, line width=2pt] (e3) -- (d4) -- (c5);
\draw[violet!50, line width=2pt] (e1) -- (e2);
\draw[violet!50, line width=2pt] (d3) -- (d4);
\draw[red!70, line width=2pt] (d1) -- (e2) -- (d3);

\end{scope}

\end{tikzpicture}

==> tables/easy.tex <==
{\tabcolsep2pt

\begin{table}
\scriptsize
\centering
\caption{MRR using the \textbf{type-matched negatives evaluation protocol} (TMN)}
\begin{tabular}{lccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{Approach} &  \multicolumn{5}{c}{FB15k-237} & \multicolumn{5}{c}{WN18RR} & \multicolumn{5}{c}{NELL-995} \\
\cmidrule(lr{.15em}){2-6} \cmidrule(lr{.15em}){7-11} \cmidrule(lr{.15em}){12-16}
& V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg  \\
\midrule
NeuralLP & .354 & .447 & .427 & .418 & .412 & .706 & .695 & .352 & .661 & .604 & .446 & .586 & .539 & .578 & .537 \\
DRUM & .399 & .490 & .448 & .454 & .448 & .708 & .696 & .352 & .661 & .604 & .483 & .621 & .606 & \textbf{.647} & .589 \\
AnyBURL & .425 & .540 & .530 & .525 & .505 & .798 & .778 & .513 & .727 & .704 & .728 & .574 & .479 & .521 & .575 \\
\midrule
GraIL & .417 & .468 & .475 & .305 & .416 & .764 & .794 & .523 & .754 & .709 & .462 & .536 & .479 & .376 & .463 \\
ConGLR & \underline{.491} & .479 & .520 & .511 & .500 & .732 & .766 & .462 & .736 & .674 & .625 & \textbf{.719} & \underline{.638} & .573 & \underline{.639} \\
COMPILE & .442 & .511 & .526 & .483 & .490 & .768 & .784 & .516 & .737 & .701 & .550 & \underline{.685} & .611 & .287 & .533 \\
SNRI & .312 & .416 & .438 & .454 & .405 & .533 & .784 & .481 & .731 & .632 & .531 & .510 & .426 & .208 & .419 \\
INDIGO & .228 & .234 & .261 & .231 & .238 & .081 & .056 & .106 & .062 & .076 & .540 & .277 & .257 & .235 & .327 \\
NodePiece & .252 & .323 & .322 & .307 & .301 & .590 & .720 & .401 & .650 & .590 & .627 & .270 & .290 & .210 & .349 \\
NBFNet & \textbf{.524} & \textbf{.602} & \textbf{.573} & \textbf{.577} & \textbf{.569} & \textbf{.895} & \textbf{.870} & \textbf{.750} & \textbf{.821} & \textbf{.834} & \underline{.745} & .665 & \textbf{.666} & \underline{.634} & \textbf{.678} \\
AStarNet & .487 & \underline{.575} & \underline{.569} & \underline{.563} & \underline{.548} & \underline{.843} & \underline{.822} & \underline{.631} & \underline{.787} & \underline{.771} & \textbf{.788} & .653 & .624 & .575 & .660 \\
RED-GNN & .402 & .514 & .551 & .545 & .503 & .799 & .807 & .600 & .768 & .743 & .732 & .618 & .588 & .387 & .581 \\
\bottomrule
 \end{tabular}
\label{tab:easy}
\end{table}
}

==> tables/easy10.tex <==
{\tabcolsep2pt

\begin{table}
\scriptsize
\centering
\caption{Hits@10 results using the \textbf{type-matched sampling evaluation protocol}. All results
were produced by us.}
\begin{tabular}{lccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{Approach} &  \multicolumn{5}{c}{FB15k-237} & \multicolumn{5}{c}{WN18RR} & \multicolumn{5}{c}{NELL-995} \\
\cmidrule(lr{.15em}){2-6} \cmidrule(lr{.15em}){7-11} \cmidrule(lr{.15em}){12-16}
& V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg  \\
\midrule
NeuralLP & .441 & .550 & .499 & .531 & .505 & .729 & .689 & .336 & .652 & .601 & .750 & .731 & .734 & .748 & .741 \\
DRUM & .446 & .556 & .497 & .533 & .508 & .729 & .689 & .336 & .652 & .601 & .755 & .745 & .752 & .758 & .752 \\
AnyBURL & .495 & .712 & .717 & .746 & .668 & .814 & .776 & .540 & .719 & .712 & .830 & .759 & .645 & .586 & .705 \\
\midrule
GraIL & .566 & .690 & .688 & .546 & .622 & .840 & .810 & .596 & .762 & .752 & .720 & .798 & .719 & .613 & .713 \\
ConGLR & \underline{.685} & .659 & .694 & .699 & .684 & .785 & .804 & .501 & .753 & .711 & .865 & \textbf{.889} & \underline{.853} & .769 & \underline{.844} \\
COMPILE & .622 & \underline{.759} & .735 & .724 & .710 & .835 & .800 & .591 & .746 & .743 & .765 & \underline{.888} & .838 & .574 & .766 \\
SNRI & .554 & .697 & .679 & .696 & .656 & \underline{.878} & .815 & .595 & .773 & .765 & .805 & .776 & .663 & .371 & .654 \\
INDIGO  & .344 & .383 & .388 & .391 & .376 & .136 & .091 & .183 & .131 & .135 & .615 & .478 & .420 & .418 & .483 \\
NodePiece & .532 & .615 & .625 & .600 & .593 & .798 & \underline{.842} & .599 & .765 & .751 & .905 & .555 & .575 & .470 & .626 \\
NBFNet & \textbf{.688} & \textbf{.794} & \textbf{.776} & \textbf{.784} & \textbf{.760} & \textbf{.941} & \textbf{.910} & \textbf{.863} & \textbf{.899} & \textbf{.903} & \underline{.970} & .861 & \textbf{.868} & \textbf{.819} & \textbf{.880} \\
AStarNet & .651 & .753 & \underline{.754} & \underline{.761} & \underline{.730} & .875 & .832 & \underline{.702} & \underline{.797} & \underline{.802} & \textbf{.975} & .828 & .794 & \underline{.775} & .843 \\
RED-GNN  & .483 & .700 & .718 & .754 & .664 & .854 & .823 & .665 & .777 & .780 & .895 & .842 & .807 & .540 & .771 \\
\bottomrule
 \end{tabular}
\label{tab:easy10}
\end{table}
}

==> tables/ilpc.tex <==
\begin{table}
\centering
\caption{MRR using the standard evaluation protocol for link prediction.}
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Approach} &  \multicolumn{4}{c}{ILPC22-S} & \multicolumn{4}{c}{ILPC22-L} \\
\cmidrule(lr{.15em}){2-5} \cmidrule(lr{.15em}){6-9}
& h@1 & h@3 & h@10 & MRR & h@1 & h@3 & h@10 & MRR \\
\midrule
NodePiece$^\dagger$ & .007 & .022 & .092 & .038 & .037 & .054 & .125 & .065 \\
NodePiece + CompGCN$^\dagger$ & .076 & .140 & .251 & .133 & .032 & .073 & .146 & .071 \\
AnyBURL Max & .146 & .249 & .374 & .220 & .184 & .271 & .351 & .241 \\
\midrule
Baseline & - & - & - & .019 & - & - & - & .009 \\
\bottomrule
 \end{tabular}
\label{tab:ilpc}
\end{table}

==> tables/standard.tex <==
{\tabcolsep2pt

\begin{table}
\scriptsize
\centering
\caption{MRR results using the \textbf{non-sampling evaluation protocol} of inductive link prediction approaches on commonly used benchmark datasets. All other results were produced by us. \textit{t/o} means that evaluation would have taken longer than 12 hours.}
\begin{tabular}{lccccr|ccccr|ccccr}
\toprule
\multirow{2}{*}{Approach} &  \multicolumn{5}{c}{FB15k-237} & \multicolumn{5}{c}{WN18RR} & \multicolumn{5}{c}{NELL-995} \\
\cmidrule(lr{.15em}){2-6} \cmidrule(lr{.15em}){7-11} \cmidrule(lr{.15em}){12-16}
& V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg  \\
\midrule
NeuralLP & .223 & .272 & .252 & .204 & .238 & .626 & .619 & .292 & .583 & .530 & .411 & .395 & .344 & .269 & .355 \\
DRUM & .284 & .356 & .289 & .280 & .302 & .627 & .620 & .280 & .582 & .527 & .402 & .383 & .387 & \underline{.393} & .391 \\
AnyBURL & .367 & .475 & .446 & .426 & .428 & .699 & .694 & .400 & .630 & .606 & .723 & .442 & .355 & .357 & .469 \\
\midrule
% GraIL & .232 & .280 & .235 & .241 & .247 & .537 & .604 & .323 & .529 & .498 & .396 & .180 & .161 & .103 & .210 \\
GraIL & .232 & .280 & .235 & \textit{t/o} & $\approx$.249 & .537 & .604 & .323 & .529 & .498 & .396 & .180 & .161 & .103 & .210 \\
ConGLR & .226 & .271 & \textit{t/o} & \textit{t/o} & $\approx$.246 & .479 & .376 & \textit{t/o} & \textit{t/o} & $\approx$.428 & .485 & .309 & \textit{t/o} & \textit{t/o} & $\approx$.397 \\
COMPILE & .265 & 306 & \textit{t/o} & \textit{t/o} & $\approx$.285 & .592 & .600 & \textit{t/o} & \textit{t/o} & $\approx$.596 & .504 & .376 & \textit{t/o} & \textit{t/o} & $\approx$.440 \\
SNRI & .159 & .252 & \textit{t/o} & \textit{t/o} & $\approx$.206 & .144 & .155 & \textit{t/o} & \textit{t/o} & $\approx$.149 & .450 & .218 & \textit{t/o} & \textit{t/o} & $\approx$.334 \\
INDIGO & .127 & .137 & .155 & .102 & .130 & .026 & .006 & .037 & .003 & .018 & .529 & .110 & .103 & .097 & .210 \\
NodePiece & .194 & .243 & .213 & .196 & .212 & .263 & .526 & .193 & .387 & .342 & .581 & .144 & .150 & .081 & .239 \\
NBFNet & \textbf{.466} & \textbf{.538} & \textbf{.494} & \textbf{.478} & \textbf{.494} & \textbf{.743} & \underline{.693} & \textbf{.452} & \underline{.641} & \underline{.632} & \underline{.737} & \textbf{.520} & \textbf{.508} & \textbf{.426} & \textbf{.548} \\
AStarNet & \underline{.427} & \underline{.514} & \underline{.483} & \underline{.469} & \underline{.473} & \underline{.730} & \textbf{.704} & \underline{.448} & \textbf{.654} & \textbf{.634} & \textbf{.769} & \underline{.501} & \underline{.476} & .294 & \underline{.510} \\
RED-GNN & .322 & .420 & .424 & .426 & .398 & .698 & .681 & .439 & .632 & .613 & .717 & .399 & .385 & .195 & .424 \\
\midrule
Baseline & .123 & .130 & .098 & .091 & .111 & .006 & .003 & .012 & .001 & .006 & .594 & .050 & .060 & .029 & .183 \\
\bottomrule
 \end{tabular}
\label{tab:standard}
\end{table}
}

==> tables/standard10.tex <==
{\tabcolsep1.6pt

%Hits@10 results using the \textbf{random sampling evaluation protocol}. $\dagger$ results were generated by us, $^\star$ results are from~\cite{grail}, other results are from the original papers.

\begin{table}
\scriptsize
\centering
\caption{Hits@10 results using the \textbf{non-sampling evaluation protocol}. All results were produced by us. \textit{t/o} means that evaluation would have taken longer than 12 hours.}
\begin{tabular}{lccccr|ccccr|ccccr}
\toprule
\multirow{2}{*}{Approach} &  \multicolumn{5}{c}{FB15k-237} & \multicolumn{5}{c}{WN18RR} & \multicolumn{5}{c}{NELL-995} \\
\cmidrule(lr{.15em}){2-6} \cmidrule(lr{.15em}){7-11} \cmidrule(lr{.15em}){12-16}
& V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg & V1 & V2 & V3 & V4 & avg  \\
\midrule
NeuralLP & .351 & .437 & .388 & .341 & .379 & .713 & .684 & .312 & .636 & .586 & .750 & .598 & .544 & .585 & .619 \\
DRUM & .385 & .468 & .410 & .403 & .417 & .715 & .680 & .310 & .635 & .585 & .755 & .554 & .585 & \underline{.591} & .621 \\
AnyBURL & .461 & .640 & .620 & .614 & .584 & .803 & .772 & .467 & \underline{.705} & .687 & .830 & .610 & .486 & .530 & .614 \\
\midrule
GraIL  & .376 & .415 & .423 & \textit{t/o} & $\approx$.404 & .729 & .744 & .406 & .675 & .638 & .685 & .310 & .336 & .219 & .387 \\
% GraIL  & .376 & .415 & .423 & 401 & .404 & .729 & .744 & .406 & .675 & .638 & .685 & .310 & .336 & .219 & .387 \\
ConGLR & .373 & .423 & \textit{t/o} & \textit{t/o} & $\approx$.398 & .566 & .688 & \textit{t/o}  & \textit{t/o} & $\approx$.627 & .810 & .512 & \textit{t/o} & \textit{t/o} & $\approx$.661 \\
COMPILE & .417 & .498 & \textit{t/o} & \textit{t/o} & $\approx$.457 & .689 & .656 & \textit{t/o} & \textit{t/o} & $\approx$.673 & .760 & .606 & \textit{t/o} & \textit{t/o} & $\approx$.683 \\
SNRI & .246 & .416 & \textit{t/o} & \textit{t/o} & $\approx$.331 & .319 & .465 & \textit{t/o} & \textit{t/o} & $\approx$.392 & .800 & .407 & \textit{t/o} & \textit{t/o} & $\approx$.603\\
INDIGO & .198 & .247 & .246 & .198 & .222 & .040 & .011 & .056 & .005 & .028 & .615 & .230 & .193 & .182 & .305 \\
NodePiece & .429 & .500 & .451 & .419 & .450 & .540 & .661 & .262 & .506 & .492 & .895 & .294 & .306 & .178 & .418 \\
NBFNet & \textbf{.617} & \textbf{.719} & \textbf{.659} & \textbf{.661} & \textbf{.664} & \textbf{.830} & \underline{.787} & \textbf{.554} & .700 & \underline{.718} & \underline{.925} & \textbf{.694} & \textbf{.688} & \textbf{.640} & \textbf{.737} \\
AStarNet & \underline{.534} & \underline{.673} & \underline{.647} & \underline{.637} & \underline{.623} & \underline{.819} & \textbf{.804} & \underline{.541} & \textbf{.736} & \textbf{.725} & \textbf{.960} & \underline{.690} & \underline{.646} & .440 & \underline{.684} \\
RED-GNN  & .420 & .590 & .582 & .600 & .548 & .774 & .776 & .532 & .696 & .694 & .840 & .582 & .553 & .301 & .569 \\
\midrule
Baseline & .351 & .384 & .253 & .211 & .300 & .005 & .002 & .022 & .000 & .007 & .835 & .124 & .129 & .049 & .284 \\
\bottomrule
 \end{tabular}
\label{tab:standard10}
\end{table}
}

==> tables/stats_old.tex <==
\begin{table}
\centering
\caption{Statistics of used benchmark datasets.}
\begin{tabular}{llcccccc}
\toprule
%\multirow{2}{*}{Dataset} & \multirow{2}{*}{Version} &  \multirow{2}{*}{Graph} & \multirow{2}{*}{Relations} & \multicolumn{2}{c}{Train} & \multicolumn{2}{c}{Valid} & \multicolumn{2}{c}{Test} \\
Dataset & Version & Graph & Relations & Entities & Train & Valid & Test \\
\midrule
\multirow{8}{*}{FB15k-237} & \multirow{2}{*}{v1} & train &  \multirow{2}{*}{180} & 1594 & 4245 & 489 & 492 \\
 & & test & & 1093 & 1993 & 206 & 205 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v2} & train &  \multirow{2}{*}{200} & 2608 & 9739 & 1166 & 1180 \\
 & & test & & 1660 & 4145 & 469 & 478 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v3} & train & 215 & 3668 & 17986 & 2194 & 2214 \\
 & & test & & 2501 & 7406 & 866 & 865 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v4} & train &  \multirow{2}{*}{219} & 4707 & 27203 & 3352 & 3361 \\
 & & test & & 3051 & 11714 & 1416 & 1424 \\
\midrule
\multirow{8}{*}{WN18RR} & \multirow{2}{*}{v1} & train &  \multirow{2}{*}{9} & 2746 & 5410 & 630 & 638 \\
 & & test &  & 922 & 1618 & 185 & 188 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v2} & train &  \multirow{2}{*}{10} & 6954 & 15262 & 1838 & 1868 \\
 & & test & & 2757 & 4011 & 411 & 441 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v3} & train &  \multirow{2}{*}{11} & 12078 & 25901 & 3097 & 3152 \\
 & & test & & 5084 & 6327 & 538 & 605 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v4} & train &  \multirow{2}{*}{9} & 3861 & 7940 & 934 & 968 \\
 & & test & & 7084 & 12334 & 1394 & 1429 \\
\midrule
\multirow{8}{*}{NELL-995} & \multirow{2}{*}{v1} & train &  \multirow{2}{*}{14} & 3103 & 4687 & 414 & 439 \\
 & & test & & 225 & 833 & 101 & 100 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v2} & train &  \multirow{2}{*}{88} & 2564 & 8219 & 922 & 968 \\
 & & test & & 2086 & 4586 & 459 & 476 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v3} & train &  \multirow{2}{*}{142} & 4647 & 16393 & 1851 & 1873 \\
 & & test & & 3566 & 8048 & 811 & 809 \\
 \cmidrule{2-8}
 & \multirow{2}{*}{v4} & train &  \multirow{2}{*}{76} & 2092 & 7546 & 876 & 867 \\
 & & test & & 2795 & 7073 & 716 & 731 \\
\midrule
\multirow{2}{*}{ILPC22-S} & & train &  \multirow{2}{*}{48} & 10230 & 78616 & - & - \\
 & & test & & 6653 & 20960 & 2908 & 2902 \\
 \midrule
\multirow{2}{*}{ILPC22-L} & & train &  \multirow{2}{*}{65} & 46626 & 202446 & - & -\\
 & & test & & 29246 & 77044 & 10179 & 10184 \\
\bottomrule
 \end{tabular}
\label{tab:stats}
\end{table}

